Neural Network Prediction of Strong Lensing Systems with Domain Adaptation and Uncertainty Quantification

Modeling strong gravitational lenses is computationally expensive for the complex data from modern and next-generation cosmic surveys. Deep learning has emerged as a promising approach for finding lenses and predicting lensing parameters, such as the Einstein radius. Mean-variance Estimators (MVEs) are a common approach for obtaining aleatoric (data) uncertainties from a neural network prediction. However, neural networks have not been demonstrated to perform well on out-of-domain target data successfully - e.g., when trained on simulated data and applied to real, observational data. In this work, we perform the first study of the efficacy of MVEs in combination with unsupervised domain adaptation (UDA) on strong lensing data. The source domain data is noiseless, and the target domain data has noise mimicking modern cosmology surveys. We find that adding UDA to MVE increases the accuracy on the target data by a factor of about two over an MVE model without UDA. Including UDA also permits much more well-calibrated aleatoric uncertainty predictions. Advancements in this approach may enable future applications of MVE models to real observational data.

==> backup_text.tex <==
% The MMD between source and target latent features is a loss tha can be minimized.

% there are no labels available the problem in which no labels are accessible for the target data at all. 
% This makes sense for SBI problems, in which one can treat the source data as the outputs of the simulator, which are intrinsically labeled, and the target domain would be future real data that one would want to deploy their model on. 
% within a deep neural network architecture. 
% $MMD_{DA}=\frac{1}{N(N-1)} \sum_{i !=j} k\left(x_{\mathrm{s}}(i), x_{\mathrm{s}}(j)\right)-k\left(x_{\mathrm{s}}(i), x_{\mathrm{t}}(j)\right)- k\left(x_{\mathrm{t}}(i), x_{\mathrm{s}}(j)\right)+k\left(x_{\mathrm{t}}(i), x_{\mathrm{t}}(j)\right),$ where the function $k$ is a linear combination of Gaussian radial basis functions. 
% Typically, latent features are the output of summarizing layers, such as convolutional layers, used before a classifier or estimator. 
% This regiment fits NPE well, as latent features are produced by the embedding network before being fed into the MAF layers. 
% We perform alignment on these vectors, specifically those output by the final convolutional layers. 



%\textcolor{red}{We use empirically and theoretically motivated priors for the physical parameter distributions in these experiments.
%For the lens-plane parameters, we use uniform priors with ranges expected for real surveys \cite{Collett_2015, bolton2008sloan}}.
% We use the \deeplenstronomy~\cite{morgan2021deeplenstronomy} software, which is built on \lenstronomy~\cite{birrer2018lenstronomy} to generate galaxy-scale strong lensing simulations of ground-based observations in a three photometric bands --- $g$, $r$, and $z$ [cite]. 
% All images have 0.263 arcsecond pixel scale to match that of DES [cite].
% The source domain data has no point spread function and no observational noise.
% The target domain data has no PSF and no photon noise, but it has readout noise drawn from a Gaussian distribution $\mathcal{N}(4,0.2)$, which is based on empirically observed DES noise parameters~\cite{PhysRevD.98.043526}. 
% Synthetic noise added to images is a combination of predicted gaussian noise due to readout noise, sky brightness, exposure time, and number of exposures, as well as poisson noise. The physics parameters are chosen for a reasonably representative range of the strong lensing parameter space. For example, $\theta_E$ is chosen to be drawn from a uniform prior $\theta_E \sim \mathcal{U}(1,3)$ arcsecond, which is typical for a galaxy-scale lens.
% Sample lenses from source and target data are given in \myfig~\ref{fig:collage}(b).


    % Model performance summaries.
    % Mean and standard deviation of the correlation $R^2$ and of the residuals for each model (\modelmve\ and \modelmveuda) as applied to the source and target domain data.


    
%The baseline requirement for a successful combination of MVE and UDA is that the \modelmveuda\ model performs comparably on the source data as the \modelmve\ model.


% we utilize a dataset of labeled, noiseless and simulated strong lenses to train a neural network for regression of lens modeling parameter $\theta_E$, using both DA and MVE. 
% This network is then applied on a more realistic, noisy dataset, that served as the target dataset for DA. 
% Regression predictions and uncertainty quantifications for both the source and target dataset are then presented, alongside the model accuracy, demonstrating the successful application of both DA and MVE to a proof-of-concept modeling challenge.


% The field of astrophysics today has been supercharged by the availability of abundant datasets of the night sky. 
% This advance has been made possible by the advent of large telescopes that regularly survey the sky to create deep maps revealing hundreds of millions of galaxies 
% % \citep{DES PAPER, DECALS PAPER, LSST PAPER}. 
% Even rare astrophysical occurrences, such as strong gravitational lensing - the morphing of galaxy structures by a chance alignment of two galaxies on the sky - are now found in large samples within these datasets due to the sheer volume of survey data, and the advent of machine-learning based detection techniques 
% % \citep{ERIK PAPER, XH PAPER}.

% Strong lensing occurs when two galaxies (at large distances from each other) are nearly aligned in our line of sight. 
% Due to the mass of the galaxy in the foreground galaxy, light from the background galaxy is bent, creating structures such as arcs and Einstein rings 
% % \citep{WALSH, HUCHRA, BOLTON}.  
% As strong lensing is caused by the effect of gravity on light, modeling the geometry of discovered strong lenses can offer important information regarding the mass structure of the foreground galaxy 
% % \citep{KOCHANEK, KOOPMANS, BOLTON, CLOWE, HUANG, JULLO},
% as well as provide us distance information, useful for understanding cosmology and the evolution of dark energy in the universe 
% % \citep{LI COLLETT, }. 
% As the number of discovered galaxy-scale strong lens candidates hover in the thousands \citep{HUANG}, constraining the dark energy evolution parameter ($w$) to a precision of 0.11 with 10,000 modeled lenses 
% % \citep{LI COLLETT, } 
% is a goal that is becoming increasingly possible.

% Modeling of strong lenses is traditionally computationally expensive, and requires the intuition of scientists in order to perform the required iteration and achieve an accurate model, even with relatively rapid modeling packages 
% % \cite{LENSTRONOMY, GIGALENS}. 
% Modeling of over O($10^3$) lenses therefore, may be infeasible for traditional approaches. Neural networks may be able to bridge this gap; they boast high-speed prediction capabilities and allow flexible distributions. 

% Performing modeling would require use of regression neural networks for parameter estimation. 
% If successful, the technique can further be expanded to other regression-based problems in astrophysics, from modeling galaxy structures \addcite{}\ to improving galaxy classification, to modeling spectra.
% Networks are already used for real classification of strong lens candidate systems from large survey datasets \addcite{}. 
% With a regression-based approach, classification can be attempted with higher fidelity.

% Two aspects prevent the broader adoption of machine learning techniques in astrophysics, however: the lack of large datasets with real labeled training data, and lack of accurate uncertainty prediction in parameter estimation. In this paper, we combine the techniques of domain adaptation (DA) and uncertainty quantification (UQ) which seek to address each of these challenges respectively. 

% Uncertainty Quantification is the...

% Domain Adaptation is the...




% \begin{enumerate}
%     \item strong lensing is an important probe of cosmology [cite]
%     \item what could be discovered or measured these data [cite]
%     \item The amount of data has growing for a long time, and will continue to grow: lots of survey data: sdss, jwst, ngrt, euclid, lsst [cite]
%     \item However, finding these objects at a high completion rate and at a low false-positive rate is long-time challenge [cite] 
%     \item the early approaches include bespoke models [cite]
%     \item Additionally modeling these objects to infer parameters is traditionally computationally highly costly.
%     \item The traditional approaches have trouble because they take so long and require extensive human intervention; why? [cite]
%     \item why neural networks can play a role.  It helps with speed of analysis and when more flexible distributions are needed. 
%     \item neural networks are used for classification now [cite]
%     \item regression neural networks can provide fast modeling to help with classification [cite], even if not parameter estimation.
%     \item where has regression been used across astronomy for2D data? [cite];   
%     \item what is missing from neural network regression in science/astronomy -- uncertainty quantification? 
%     \item define UQ
%     \item has UQ been used in the past for neural network regression in science/astronomy, including strong lensing? [cite]
%     \item what is missing from neural network regression in science/astronomy -- domain adaptation? 
%     \item define DA and domain shift
%     \item has DA been used in the past for neural network regression in science/astronomy, including strong lensing? [cite]
%     \item How does this paper build on prior work in each area?
%     \item How does this paper set the stage for a longer-term goal?
%     \item What do we do in this paper specifically?
% \end{enumerate}


% provide a wealth of data on galaxy-scale strong lensing systems --- e.g., the Dark Energy Survey~\cite{the_dark_energy_survey_collaboration_dark_2005, flaugher_dark_2015},  Hyper Suprime-Cam~\cite{2022PASJ...74..247A, 2023PhRvD.108l3520M}, the Kilo-Degree Survey (KiDS)~\cite{2013ExA....35...25D, 2019A&A...625A...2K}, the Rubin Observatory Legacy Survey of Space and Time~\cite{ivezic_lsst_2019}, Euclid~\cite{2024arXiv240513491E}, JWST~\cite{schaerer_first_2022, brummel-smith_inferred_2023}, and the Nancy Grace Roman Telescope~\cite{eifler_cosmology_2021, la_plante_prospects_2023, wang_high_2022-1} --- are



% \reducethisforspace{
% To generate realistic colors, each simulated lens galaxy is assigned a redshift $z_l < 0.7$, and each simulated background galaxy a redshift $1.27< z_s < 2$ according to the photo-$z$ distribution of the DES Y3 Gold Catalog ~\cite{SN2021, zaborowski_identification_nodate}. 
% Each simulated galaxy is then assigned a random color from a real galaxy at that redshift~\cite{Dey2019}.
% % using the Legacy Surveys DR10 catalog, which partly uses DES imaging~\cite{Dey2019}. 
% To ensure that each lens galaxy is visible but not saturated, we use a lower limit on the apparent magnitude for all bands $\{m_g, m_r, m_z\} > 17.5$ and an upper limit for any one of the bands $\{m_g, m_r, m_z\} < 21$. 
% For the background galaxy, we use the constraints of~\cite{zaborowski_identification_nodate}: $\{m_g, m_r, m_z\} > 17.5$ and $m_g < 22$. 
% Redshifts are independent of the lensing configuration and are solely used for realistic galaxy colors.
% }




% Finally, we studied model stability across five differently initialized models. The median residuals are consistent with the “Selected” model (Table 1(c,d)). Across runs, the \modelmve{} model  performs unpredictably on target data  (NLL min: -2.66, NLL max: 15503.4) . This is unlike the \modelmveuda{} model which retains consistent performance (NLL min: -2.06, NLL max: -2.44). 
% Please see the \mytable~\ref{table:performance_appendix} in the appendix for the other models' residuals and uncertainties.
% There is variation in performance among the models for each diagnostic. 
% On \datatarget{} data, the \modelmveuda{} model has five times higher uncertainties ($\sigmaalmean{}~0.05$\myarcsec{}) but is better calibrated than the \modelmve{} model on \datatarget{} data and similarly calibrated as the \modelmveuda{} model on \datasource{} data.
% }


% MVE and UDA techniques each present well-known challenges for training toward convergence. 
% This is apparent from fluctuating loss functions for MVE and long times to convergence for UDA~\cite{Seitzer2022}.
% There are also some well-studied strategies for achieving fit/training convergence and stability across training runs \addcite{}.
% We experimented with many hyperparameter choices for batch size, learning rate, and optimizer.
%We found that the model achieved the highest performance when we selected the model weights when the NLL loss on the \datasource{} data reached its minimum value within 150 epochs of training. 


% \needsediting{This variation of NLL is used instead of the original because the latter's strong dependence on the gradients of the predictive variance causes undersampling of poorly predicted data points~\cite{Seitzer2022}. }
 % The gradient of the original NLL loss is highly dependent on the variances predicted. 
% For high-error points, the gradient becomes small, causing them to be effectively undersampled. $\beta$-NLL resolves this by multiplying a variance-reweighting term $\sigma^{2\beta_\textrm{NLL}}$~\cite{Seitzer2022}.  

% There are three standard types of uncertainty that are considered in the use of neural networks: aleatoric (intrinsic data uncertainty), epistemic (model uncertainty), and domain (difference between data domains)~\cite{farahani_brief_2020}.


% $L_{\mathrm{Tot}} = \mathcal{L}_{\beta-\mathrm{NLL}}(\betanll) + \alpha_{\mathrm{UDA}}* L_{\mathrm{UDA}}$,  
% both the convolutional and dense layers of the network.


% We use the \deeplenstronomy~\cite{deeplenstronomy} software, built on \lenstronomy~\cite{lenstronomy:2018, lenstronomy:2021}, to simulate ground-based telescope images of galaxy-scale strong lenses.
%%%% image settings


%%%% noise parameter distributions for the domain shift
% https://github.com/deepskies/DAUQ_LensModeling/blob/main/src/sim/configs/multiband_paper_source_final.yaml
% https://github.com/deepskies/DAUQ_LensModeling/blob/main/src/sim/configs/multiband_paper_target_final.yaml


% The distributions are available in  \deeplenstronomy{}\~\cite{deeplenstronomy}. 
%%%% data set split

% Sample lenses from source and target data are shown in \myfig{}~\ref{fig:latent}(a).

% Therefore, the \modelmveuda{} is slightly more biased but has better calibrated uncertainties and the \modelmve{} when they are applied to source data.
